Generating Interactive WebSocket Applications in TypeScript

Advancements in mobile device computing power have made interactive web applications possible, allowing the web browser to render contents dynamically and support low-latency communication with the server. This comes at a cost to the developer, who now needs to reason more about correctness of communication patterns in their application as web applications support more complex communication patterns. Multiparty session types (MPST) provide a framework for verifying conformance of implementations to their prescribed communication protocol. Existing proposals for applying the MPST framework in application developments either neglect the event-driven nature of web applications, or lack compatibility with industry tools and practices, which discourages mainstream adoption by web developers. In this paper, we present an implementation of the MPST framework for developing interactive web applications using familiar industry tools using TypeScript and the React.js framework. The developer can use the Scribble protocol language to specify the protocol and use the Scribble toolchain to validate and obtain the local protocol for each role. The local protocol describes the interactions of the global communication protocol observed by the role. We encode the local protocol into TypeScript types, catering for server-side and client-side targets separately. We show that our encoding guarantees that only implementations which conform to the protocol can type-check. We demonstrate the effectiveness of our approach through a web-based implementation of the classic Noughts and Crosses game from an MPST formalism of the game logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{12}
\providecommand{\publicationstatus}{S. Balzer, L. Padovani (Eds.): Programming Language Approaches\\
to Concurrency- \& Communication-cEntric Software (PLACES 2020)\\
EPTCS 314, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.314.2}{10.4204/EPTCS.314.2}}
\pdfoutput=1

